Suspended thin-film lithium niobate modulator for broadband mid-infrared light modulation and frequency comb generation

The mid-infrared (MIR) spectral regime is central to applications including remote sensing, precision spectroscopy, higher harmonic generation, and free-space optical communication. However, coherent and broadband MIR modulation remains challenging owing to high optical loss, limited bandwidth, and large drive voltages in existing platforms. Here, we overcome these challenges by deploying a suspended thin-film lithium-niobate (TFLN) based electro-optic (EO) platform co-designed with high-performance traveling-wave microwave (MW) electrodes. We demonstrate a record-low Vpi,DC of 2.3 to 4.3 V over a broadband MIR bandwidth from 2.4 to 3.6 um, and a 2.7 dB EO bandwidth of 40 GHz (extracted 3 dB bandwidth of 50 GHz), yielding a figure of merit of 17.4 GHz/V, more than an order of magnitude higher than the state of the art. We demonstrate, for the first time, high-frequency Vpi,MW of 4.5 to 6.5 V in the 25 to 35 GHz range, and frequency-agile MIR EO frequency comb generation with a 10 dB optical bandwidth over 0.8 THz using a suspended phase modulator of 4 cm active modulation length. We further validate the platform in a free-space optical communication link. Our results establish a monolithic MIR photonic platform capable of powerful EO modulation and spectral synthesis, and represent a significant step toward reconfigurable MIR sensing and communication systems on chip.

==> Figure.tex <==

% Language setting
% Replace `english' with e.g. `spanish' to change the document language
\usepackage[english]{babel}


% Set page size and margins
% Replace `letterpaper' with `a4paper' for UK/EU standard size
\usepackage[letterpaper,top=2cm,bottom=2cm,left=3cm,right=3cm,marginparwidth=1.75cm]{geometry}

% Useful packages
\usepackage{amsmath}
\usepackage{soul}
\usepackage[colorlinks=true, allcolors=blue]{hyperref}

% Put these in your preamble for table
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage{makecell}
\usepackage{siunitx}
\usepackage{caption}
\usepackage{array}
\usepackage{longtable}
\usepackage{geometry} % optional, for wider margins if needed
\usepackage{graphicx}   % for \resizebox
\usepackage{authblk}
\usepackage{cite}

\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{Figures/Figure1_v1.jpg}
\caption{\label{fig:figure1} \textbf{Monolithic mid-infrared optoelectronic platform on thin film lithium niobate (TFLN).} (a) Air-suspended MIR traveling-wave-based amplitude and phase electro-optic modulators on the TFLN. Inset shows the cross-sectional view of the optical layer which consists of a ridge TFLN waveguide sitting on oxide-on-Si substrate. The oxide layer is removed underneath the waveguide area through air holes on the TFLN slab layer etched via a second etching process. High performance optoelectronic interface in the MIR would enable high-bandwidth data links via free space communication (b) and frequency-agile EO frequency combs for molecular spectroscopy (c). (d) Photographic image of the fabricated MIR modulator chip on 800-nm X-cut TFLN. (e) Scanning-electron-microscopy (SEM) image of suspended photonic waveguides and coplanar microwave transmission line. Segmented slow-wave electrode design (zoom in, right) is applied to reduce the microwave loss and achieve impedance matching and velocity matching with optical field while compatible with a low optical propagation loss. Air hole arrays are optimized and placed between the metal segments for releasing the adjacent photonic waveguides. (f) Cross section of the suspended device where the metal gap (g), waveguide height ($h_{LN}$), slab thickness ($h_{slab}$), metal thickness ($h_{metal}$), waveguide width ($w_{0}$), the air gap under the waveguide ($h_{air}$) and the segmented electrode parameters (s , t, r , l ) are 6.5, 0.8, 0.25, 0.8, 4, 4.7 $\mu$m, and (0.5, 6.5, 0.5, 45) $\mu$m, respectively. The SEM image of the waveguide facet is shown. The simulated transverse-electric optical mode profile at 3 $\mu$m is plotted.}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{Figures/Figure2_v1.jpg}
\caption{\label{fig:figure2}| \textbf{Characterization of near-DC half-wave voltage $V_\pi$ of a 2-cm-long air-suspended amplitude modulator.} (a) Optical microscope images. Two optical path in the AM have a different length of 21 $\mu$m to enable bias point tuning via varying the optical wavelength. (b) Normalized optical transmission as a function of applied voltage at the different MIR wavelengths as well as at the 1.55 $\mu$m in the NIR. The measured half-wave voltage ($V_\pi$) at 100 kHz is 2.3 - 4.26 V across the optical span from 2.4 $\mu$m to 3.6 $\mu$m, which indicates approximately linear dependence of the optical operational wavelength. In addition, the suspended AM device is measured across more than an octave optical bandwidth with a half-wave voltage of 1.8 V at 1.55 $\mu$m. (c) Comparison of  $V_\pi$ with other MIR EO platforms. The LN amplitude modulator shows the lowest  $V_\pi$  as well as  $V_\pi$⋅L of 4.6 V⋅cm at 2.4 $\mu$m and 8.6 V⋅cm at 3.6 $\mu$m.}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{Figures/Figure3_v1.jpg}
\caption{\label{fig:figure3} \textbf{Characterization of the MIR modulator up to 40-GHz microwave frequencies.} (a) Measured microwave loss on the segmented co-planar electrodes before and after air suspension. Segmented travel-wave electrodes combined with air suspension lead to a reduced MW propagation loss of 2.75 dB/cm at 40 GHz and an ohmic-loss-limited slope of 0.26 dB/cm/$GHz^{0.5}$ , which is comparable to the loss slope of the best NIR LN modulators reported\hl{[HL optica paper]}. (b) Measured electrical transmission $S_{21}$ and reflection $S_{11}$ spectrum. The measured reflection is below 25 dB from 2 - 40 GHz range indicating a well-matched impedance to 50 $\Omega$. (c) Measured MW phase index, which matches well with the optical group index based on the air-suspended TFLN waveguide (dashed line). (d) Microwave $V_\pi$ and the corresponding electro-optic response, referenced to the performance at 2 GHz.  Microwave $V_\pi$ are measured to be 5 V at 27 GHz and 5.26 V at 34 GHz for a 2-cm-long EO AM at the optical wavelength of 2.7 $\mu$m. The microwave $V_\pi$ is extracted via the optical spectrum from the AM under MW driving. The measurement results match with the simulation based on the measured S parameters in (a). Electro-optic response scales inversely with the square of the microwave $V_\pi$ and drops 2.7 dB at 40 GHz MW frequency which is the frequency limit of our signal generator while the extracted 3-dB EO BW is 50 GHz (dashed line). (e) Comparison of the modulator figure of merit, defined as the ratio between the 3-dB EO bandwidth (BW) and the near-DC $V_\pi$. The AM in our work demonstrates significantly higher BW/$V_\pi$ values of 17.4 GHz/V, as compared to the literature values (the dashed lines indicate constant BW/$V_\pi$ values). }
\end{figure}


\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{Figures/Figure4_v1.jpg}
\caption{\label{fig:figure4} \textbf{Frequency-agile MIR electro-optic frequency combs based on an integrated recycled phase modulator.} (a) Microscopic image of the suspended double passing phase modulator with the total modulation length of 4 cm. (b) Broadband EO frequency comb generation using the same PM device at two different MIR wavelengths of 2.36 $\mu$m and 2.7 $\mu$m. Total modulation indexes of 4.2 $\pi$  and 4 $\pi$ at MW driving frequencies of 27.2 and 29.2 GHz were measured at 2.36 $\mu$m and 2.7 $\mu$m pump wavelength, respectively. This corresponds to a 10-dB optical bandwidth of 0.8 THz.}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{Figures/Figure5_v1.jpg}
\caption{\label{fig:figure4} \textbf{Experimental MIR communication link using an air-suspended TFLN intensity modulator.} (a) Experimental setup for measuring the communication link at 2.7 $\mu$m wavelength. OPO: optical parametric oscillator, HWP: half-wave plate, AWG: arbitrary waveform generator, MCT detector: mercury cadmium telluride detector, DSO: digital storage oscilloscope. (b) Measured BER curve versus transmitted optical power for 1.5-Gbaud on-off keying (OOK) signal. (c-f) Experimental results of eye diagram, BER values, and Q-factors of (c) 1.5-Gbaud OOK, (d) 0.5-Gbaud PAM-4, (e) 1.5-Gbaud PAM-4, (f) 0.5-Gbaud PAM-8. The achievable data rate is limited by the 3-dB bandwidth of our MIR detector (1 GHz). }
\end{figure}



\begin{table*}[t]
\centering
\caption{Comparison of mid-infrared electro-optic modulators.}
\tiny
\renewcommand{\arraystretch}{0.9}
\setlength{\tabcolsep}{1pt}

\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l l l l c c c c c c c l c}
\toprule
\makecell{\textbf{Wave-}\\\textbf{length} \\\textbf{(\boldmath{$\mu$m})}} &
\makecell{\textbf{Platform-}\\\textbf{design}} &
\makecell{\textbf{Scheme}} &
\makecell{\textbf{Functi-}\\\textbf{onality}} &
\makecell{\textbf{L}\\\textbf{(cm)}} &
\makecell{\textbf{$V_{\pi,DC}$}\\\textbf{(V)}} &
\makecell{\textbf{MW}\\\textbf{$V_\pi$ (V)}} &
\makecell{\textbf{Optical}\\\textbf{loss}\\\textbf{(dB/cm)}} &
\makecell{\textbf{MW}\\\textbf{loss}\\\textbf{(dB/cm)}} &
\makecell{\textbf{3-dB EO}\\\textbf{BW}} &
\makecell{\textbf{3-dB EO}\\\textbf{BW per} \\\textbf{ $V_{\pi,DC}$}\\\textbf{ (GHz/V)}} &
\makecell{\textbf{Application}} &
\textbf{Ref.}\\
\midrule

\makecell{2.4\\--3.6} &
\makecell{Air-suspended\\TFLN, MZI} &
Pockels &
\makecell{AM, \\PM, \\combs} &
2 &
\begin{tabular}{@{}c@{}}2.3\\ @2.4~$\mu$m \\ 4.2 \\@3.6~$\mu$m\end{tabular} &
\begin{tabular}{@{}c@{}}4.5\\@25~GHz\\6.5~V \\@35~GHz\end{tabular} &
\begin{tabular}{@{}c@{}}3.0 \\@2.4~$\mu$m \\ 3.5 \\@ 3.6~$\mu$m\end{tabular} &
\begin{tabular}{@{}c@{}}2.75 \\ @40~GHz\end{tabular} &
{\begin{tabular}{@{}c@{}}\makecell{50~GHz \\(extrap.) }\end{tabular}} &
17.4 &
\makecell{EO comb of \\ 0.8~THz span\\Mod index of 4\pi\\OOK@10~Gbit/s\\ PAM8@1.5~Gbit/s} &
\makecell{\textbf{This}\\ \textbf{work}} \\
\midrule

\makecell{2.5} & \makecell{TiO$_2$-on-LN, \\ WG}& Pockels & AM & NA & NA & NA & NA & NA & NA & NA & NA &15 \\
\makecell{2.6} & \makecell{BTO-on-oxide, \\WG} & Pockels & AM & 0.2 & 55 & NA & 2.3 & NA & NA & NA &NA & 21 \\
\makecell{3.39} & \makecell{Si-on-LN, \\MZI} & Pockels & AM & 0.5 & 52 & NA & \makecell{2.5} & NA & $>$23~kHz$^{a}$ & NA &NA & 14 \\
\makecell{3.39} & \makecell{Ti-diffused LN,\\ MZI} & Pockels & AM & 0.8 & 31 & NA & NA & NA & 1.8~GHz & 0.058 & NA & 16 \\
\makecell{3.78} & \makecell{Si-on-LN, \\MZI} & Pockels & AM & 0.6 & 20.8 & NA & \makecell{4.5} & NA & 5~MHz & 0.00024 &NA & 13 \\
\makecell{3.8} & \makecell{Si-on-SiO$_2$, \\MZI} & TO & AM & NA & NA & NA & 3.5 & NA & $>$23.8~kHz$^{a}$ & NA & NA & 12 \\
\makecell{3.85\\--4.1} & \makecell{BP-Si-on-SiO$_2$, \\WG} & EA$^{b}$ & AM & NA & NA & NA & NA & NA & $>$60~kHz$^{a}$ & NA & NA & 17 \\
\makecell{3.8} & \makecell{Ge-on-Si, \\MZI/EAM} & Cl/CA & AM & 0.1 & 4.7 & NA & NA & NA & 60~MHz & 0.013 & OOK@60~MHz & 20 \\
\makecell{3.72\\--3.8} & \makecell{Si-on-oxide, \\MZI/EAM} & Cl/CA & AM & NA & NA & NA & 11.5 & NA & NA & NA & OOK@125~Mbit/s & 18 \\
\makecell{3.95\\--4.3} & \makecell{TFLN-on-Al$_2$O$_3$, \\MZI} & Pockels & AM & 0.8 & 28 & NA & 2.2 & NA & 20~GHz & 0.71 & OOK@10~Gbit/s & 24 \\
\makecell{3.3\\--3.8} & \makecell{Air-clad TFLN, \\cavity} & Pockels & AM & 0.15 & 51 & NA & 4 & NA & NA & NA & NA & 23 \\


\bottomrule
\end{tabular}
\end{adjustbox}
\caption*{\footnotesize 
ER: extinction ratio; EO: electro-optic; TO: thermo-optic; 
BP: black phosphorus; EAM: electro-absorption modulator; 
CI: free carrier injection; CA: free carrier absorption. Mod: modulation\\[2pt]
$^{a)}$ The measured bandwidths are limited by the PD speed.\\
$^{b)}$ The electric field changes the carrier distribution in BP, affecting its absorption.}

\end{table*}

